Modeling Category-Selective Cortical Regions with Topographic Variational Autoencoders

Category-selectivity in the brain describes the observation that certain spatially localized areas of the cerebral cortex tend to respond robustly and selectively to stimuli from specific limited categories. One of the most well known examples of category-selectivity is the Fusiform Face Area (FFA), an area of the inferior temporal cortex in primates which responds preferentially to images of faces when compared with objects or other generic stimuli. In this work, we leverage the newly introduced Topographic Variational Autoencoder to model the emergence of such localized category-selectivity in an unsupervised manner. Experimentally, we demonstrate our model yields spatially dense neural clusters selective to faces, bodies, and places through visualized maps of Cohen's d metric. We compare our model with related supervised approaches, namely the Topographic Deep Artificial Neural Network (TDANN) of Lee et al., and discuss both theoretical and empirical similarities. Finally, we show preliminary results suggesting that our model yields a nested spatial hierarchy of increasingly abstract categories, analogous to observations from the human ventral temporal cortex.

==> sections/checklist.tex <==

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{Checklist}

% \begin{enumerate}

% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerTODO{}
%   \item Did you describe the limitations of your work?
%     \answerTODO{}
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerTODO{}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerTODO{}
% \end{enumerate}

% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerTODO{}
%     \item Did you include complete proofs of all theoretical results?
%     \answerTODO{}
% \end{enumerate}

% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerTODO{}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerTODO{}
%     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerTODO{}
%     \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerTODO{}
% \end{enumerate}

% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerTODO{}
%   \item Did you mention the license of the assets?
%     \answerTODO{}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerTODO{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerTODO{}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerTODO{}
% \end{enumerate}

% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerTODO{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerTODO{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerTODO{}
% \end{enumerate}

% \end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/introduction_old.tex <==

\section{Introduction}


Domain-selectivity is observed throughout the cerebral cortex. At a high level it describes the observation that certain localized regions of the cerebral cortex have been measured to respond preferentially to specific stimuli when compared with a set of control images or a generic 'object' class. Examples of domain specific areas in the visual stream include the Fuisform Face Area (FFA) \cite{ffa}, the Parahippocampal Place Area (PPA) \cite{ppa}, and the Extrastriate Body Area (EBA) \cite{ppa} which respond selectively to faces, places, and bodies respectively. In addition to domain specificity, many visual areas have been shown to be functionally selective as well, meaning that localized areas exhibit specific functional properties such as a selectivity to directional motion in the middle temporal area (MT/V5) \cite{MT}, or control of spatial attention and saccadic eye movements in regions of the intraparietal sulcus (IPS1 \& IPS2) \cite{PrinciplesOfNeuralScience}. 
Such selectivity has been measured directly through fMRI and neural recordings, and more indirectly through observational studies of patients with localized cortical damage. 

In interpreting these observations, one may naturally wonder why neurons functionally specialize at all, regardless of spatial location, or equivalently, why shouldn't all neurons be used simultaneously to code for all observations? One potential answer to this question comes from the principle of "redundancy reduction" or the efficient coding hypothesis \cite{barlow}. Taking inspiration from Information Theory, the principle describes the idea that an optimal coding scheme is one which minimizes the transmission of redundant information. Applied to neural systems, this describes the ideal network as one which has statistically maximally independant activations -- yielding a form of specialization. Although this is certainly not entirely true of the brain (e.g. there is known redundancy for the purposes of robustness and error correction), the idea served as a guiding principle which provided the impetus for computational frameworks such as Sparse Coding \cite{olshausen} and Independant Component Analysis (ICA) \cite{hyvarinen, common, sjnowski}. As we will discuss in Section \ref{sec:TVAE}, the Topographic Variational Autoencoder discussed in this work is highly related to ICA, and thus the observed specialization of neurons may indeed derive its theoretical basis from such a principle. 

Given such a potential explanation for the emergence of functional specialization of individual neurons, what then could we expect to be the driving force behind the topographic organization and localization of densely specialized 'areas'? In the neuroscience literature, the idea of 'wiring length minimization' has been proposed as one solution \cite{wiringlength}. Briefly, the idea posits that brain strives to reduce the cumulative length of neural connections in order to reduce the costs associated with 
% the maintenance of 
such connections. %, to increase the speed of communication, as well as to reduce total brain volume. 
Further, it is assumed that neurons which are functionally similar are likely to be those which are the most densely interconnected, and thus  combined, these ideas yield a topographic organization of functional specialization. 

In the machine learning literature, an alternative computational explanation for topographic organization has been proposed, again derived from the aforementioned principle of redundancy reduction. Specifically, in the framework of ICA, it was shown that features learned by linear ICA models were not entirely independant, but indeed contained correlation of higher order statistics. In response, \emph{Topographic Generative Models} were introduced, proposing to model these residual dependencies as a function of distance in a spatial domain. In other words, topographic generative models pre-define a spatial layout of latent variables, and subsequently place a prior over activations which encourages spatial locality of neurons with higher order dependencies. 

In this work, we demonstrate that the Topographic Variational Autoencoder (TVAE), a modern instantiation of a topographic generative model, can indeed be seen to yield localized domain-selective areas entirely unsupervised in modern deep neural network architectures. We validate this domain selectivity quantitatively through the visualization of the Cohen's d' selectivity metric for different image classes, showing selective clusters for faces, bodies, and places. We compare our model with the supervised wiring cost proxies of Dicarlo et al \cite{TDANN} and demonstrate qualitatively similar results, without the need for class level supervision. Finally, we show preliminary results indicating that our model contains a nested spatial hierarchy of increasingly abstract categories, similar to those observed in the human ventral temporal cortex \cite{hierarchy}.



==> sections/relatedwork.tex <==


\paragraph{Related Work} Recently, a number of models of topographic organization in the visual system have been developed leveraging modern deep neural networks. \citet{VTCSOM} demonstrated the emergence of category-selective regions, as well as a nested spatial hierarchy of selectivity, by training a self-organizing map (SOM) on-top of dimensionality-reduced convolutional features. Concurrently, \citet{Blauch2021} developed the Interactive Topographic Network (ITN), inducing local correlation through locally-biased excitatory feedforward connections. Most related to this work, \citet{TDANN} demonstrated that a biologically derived proxy for wiring length cost, namely a local spatial correlation function (see Section \ref{appendix:spatial_loss}), can be added to existing supervised deep neural networks, yielding topographic organization and the emergence of localized category-selectivity in the final fully connected layers of an Alexnet architecture \cite{alexnet}. They denote this model the TDANN, and we provide a re-implementation in this work as a baseline for comparison. Our work differs from thes



\section{Related Work}
\paragraph{Topographic Deep ANN} In recent work, Dicarlo et al. \cite{TDANN} demonstrated that a biologically derived proxy for wiring length cost, namely a local spatial correlation function, can be successfully added to supervised deep neural networks, yielding topographic organization and the emergence of domain specific areas in the final fully connected layers of an Alexnet architecture \cite{alexnet}. Specifically, they demonstrate the emergence of a 'face area', and quantitatively compare its properties (such as relative size and purity) with face areas measured in macaque monkeys. Interestingly, the proposed wiring length proxy turns out to be based on the same underlying statistical property as the topographic generative models described in this work, namely local correlation. This suggests that these ideas may not be mutually exclusive, and hints at a potential fundamental connection between wiring length minimization and a generative modeling perspective of the brain. Our work differs from the work of \cite{TDANN} in that our model is trained without supervised class labels while still yielding class-specific clusters. Furthermore, we show preliminary results demonstrating how the entire model can be trained end-to-end unsupervised, something which is not possible the the framework of the TDANN.  
% TDANN also showed that model face patches were predictive of macaque face neurons, andfurther showed dense interconnectivity of the patches, and invariance to faces in higher layers. We couldnt do these because... 



\paragraph{SOM} SOMs have been used to model spatial organization of early visual cortex such as orientation and direction of motion. cite 34,35 dicarlo. Unfortunately these models do not scale to high dimensional inputs.

\paragraph{VTC-SOM} Concurrently with this work, Zhang et al. \cite{vtcsom} demonstrated the emergence of similar domain-selective regions by training a self-organizing map (SOM) on-top of dimensionality-reduced pre-trained Alexnet features. They additionally demonstrate topographic organization of higher-level functional specificity to abstract categories such as animacy and real-world size, and further show that these can smoothly deformed to qualitatively match results from human fMRI data. Our model differs from the SOM of \cite{vtcsom} in that it is a probabalistically based generative model which explicitly formulates a properly normalized density over the input data, and further explicitly maximizes the probability of the data through a lower bound rather than a heuristic learning algorithm. This allows the TVAE to simultaneously perform dimensionality reduction and feature extraction while scaling to train entire deep neural networks, feats unachievable with the SOM.
% Furthermore, we use a d' threshold of 0.85 instead of 0.5 used in the VTC-SOM work. 

\paragraph{Emergence of Functional Specialization} Recently, empirical studies have further validated the idea that sufficiently deep artificial neural networks naturally learn distinct and largely separate sets of features for certain domains such as faces and objects. Specifically, the work of Dobbs et al. \cite{dobbs}, showed that feature maps in the later layers of deep convolutional neural networks can be effectively segregated into object and face features such that lesioning one set of feature maps does not significantly impact performance of the network on classification of the other data domain. Such experiments suggest that the specialization of neurons may simply be an optimal method for representing the natural statistics of the underlying data when given a sufficiently powerful feature extractor, and can thus be similarly seen as a form a efficient coding. 

